Hardness Amplification of Optimization Problems

In this paper, we prove a general hardness amplification scheme for optimization problems based on the technique of direct products. We say that an optimization problem $\Pi$ is direct product feasible if it is possible to efficiently aggregate any $k$ instances of $\Pi$ and form one large instance of $\Pi$ such that given an optimal feasible solution to the larger instance, we can efficiently find optimal feasible solutions to all the $k$ smaller instances. Given a direct product feasible optimization problem $\Pi$, our hardness amplification theorem may be informally stated as follows: If there is a distribution $\mathcal{D}$ over instances of $\Pi$ of size $n$ such that every randomized algorithm running in time $t(n)$ fails to solve $\Pi$ on $\frac{1}{\alpha(n)}$ fraction of inputs sampled from $\mathcal{D}$, then, assuming some relationships on $\alpha(n)$ and $t(n)$, there is a distribution $\mathcal{D}'$ over instances of $\Pi$ of size $O(n\cdot \alpha(n))$ such that every randomized algorithm running in time $\frac{t(n)}{poly(\alpha(n))}$ fails to solve $\Pi$ on $\frac{99}{100}$ fraction of inputs sampled from $\mathcal{D}'$. As a consequence of the above theorem, we show hardness amplification of problems in various classes such as NP-hard problems like Max-Clique, Knapsack, and Max-SAT, problems in P such as Longest Common Subsequence, Edit Distance, Matrix Multiplication, and even problems in TFNP such as Factoring and computing Nash equilibrium.

==> related.tex <==


\subsection{Related Works}\label{sec:related}

In this subsection, we briefly summarize some related works on hardness amplification. The interested reader is directed to the survey of Bogdanov and Trevisan \cite{BTsurvey} for more details on most of the below works.

\paragraph{\EXP.} Impagliazzo and Wigderson \cite{IW97} showed how to obtain a Boolean function of high average-case hardness, starting with a Boolean function of high worst-case hardness. The first step was the
low-degree polynomial encoding of the truth table of a given worst-case hard Boolean function, as
in \cite{BFNW93}. This produced a Boolean function that is ``mildly'' hard on the average: any small
circuit can compute the new function correctly on at most $1 - 1/poly(n)$ fraction of all n-bit inputs.
The second step was the amplification of the average-case hardness via the derandomized version
of Yao’s XOR Lemma, so that no small circuit can compute the resulting function on more that $1/2 + 1/2^{\Omega(n)}$ fraction of all n-bit inputs.
Sudan, Trevisan, and Vadhan \cite{STV01} show that the first step alone, with a different choice
of parameters, already gives the desired high average-case hardness, and so no further hardness
amplification is needed.  


\paragraph{\#\P.} \cite{L89,CPS99}

\paragraph{\NP.} \cite{Tre05,O04,HVV06,BT06,GST07,GT07,GG11}

\paragraph{\P.} \cite{BRSV17,GR18,GR17}

\paragraph{Cryptography.} Hardness amplification has also been studied with a more direct focus on crytography, for example in \cite{Y82,GILVZ90,BR13}, the authors study hardness amplification for one-way functions. 



More than two decades ago, Lipton \cite{L89} indeed  proved the above type of (utopic) theorem for the case of the permanent function: They show that the  permanent 
function can be computed on the worst case by deterministic polynomial time algorithm, then permanent can be computed by a probabilistic polynomial time algorithm. This is proven by showing that the permanent function is self-reducible. In fact, the result was further sharpened by Cai, Pavan and Sivakumar~\cite{CPS99}.

For the class $\EXP$, Trevisan and Vadhan~\cite{TV07} almost proved the dream theorem against uniform probabilistic algorithms. They show that the existence of a family $\set {f_n}\in \EXP$ which cannot be solved in the worst case by algorithms running in time $t(n)$ implies:
the existence of a different family $\set {g_n}\in \EXP$ that cannot be solved by a $t'(n)$-time algorithms on $1/2+\epsilon(n)$-fraction of random instances, where: $t'(n)\in \poly(t(n))$ and $\epsilon(n)=t(n)^{\Omega(1)}$. Here $g_n\neq f_n$ but rather obtained by encoding $f_n$ using a locally decodable code.
%◦ noticeably better than guessing the answer at random.


For the class $\NP$ we are far from proving the dream theorem, and we are facing some barriers while trying to convert worst case $\NP$-hardness into average case (see e.g. \cite{BT06}). The state of the art hardness against non-uniform circuits is due to Heally et al.~\cite{HVV06}. They show that assuming If there exists $ f\in \NP$ on which every  circuit of size $s(n)$ fails to compute $f$ on  $1/\text{poly}(n)$ fraction of inputs then: there exists  $ g \in \NP$ on which any circuit of size $s'(n)$ fail to compute $g$ on at least $1/2 -1/s'(n)$ fraction of inputs. In the uniform case, Trevisan~\cite{Tre05} showed similar result under the stronger assumption that every $t(n)$-time algorithm fails on at least $1/\text{poly}(\log n)$ fraction of inputs. The idea of these results is encoding the function $f$ by taking multiple instances of $f$ and aggregate them by applying a monotone function on top of it.

The last class we survey is the class of problem in $\P$. In the context of fine grained complexity researchers study  the exact complexity of problems in $\P$, attempting to pinpoint the exact running time neded for solving problems (and distinguishing, say, linear-time from quadratic-time and cubic-time). A long line of research studies (conditional) worst case hardness results for problems in $\P$. Naturally, one can ask whether these results are still applicable in the average case. 

Goldreich and Rothblum~\cite{GR18} proved a worst case to an average case reduction for the problem of counting $t$-cliques against $\tilde O(n^2)$-time uniform algorithms. Ball et al.~\cite{BRSV17} show that there exist (almost linear-time) reductions from the worst-case of several \textit{natural} problems in $\P$, to the average-case of some other (but less natural) problems in $\P$.

